Visual Script and Language Identification

In this paper we introduce a script identification method based on hand-crafted texture features and an artificial neural network. The proposed pipeline achieves near state-of-the-art performance for script identification of video-text and state-of-the-art performance on visual language identification of handwritten text. More than using the deep network as a classifier, the use of its intermediary activations as a learned metric demonstrates remarkable results and allows the use of discriminative models on unknown classes. Comparative experiments in video-text and text in the wild datasets provide insights on the internals of the proposed deep network.

==> tbl_siw10.tex <==
\begin{table}
\label{tbl:siw10}
\centering
\caption{Accuracy \% on the SIW 10 Scene-text Dataset}
\begin{tabular}{l|ccc|ccc}
\hline
Language & MSPN & CNN & LLC & Layer 1 & Layer 2 & NN Layer 3 \\
& & Patch & & 1NN  & 1NN  & ANN Output\\
\hline 
Arabic & 98.6 & 94.7 & 97.0 & & & \\
Chinese & 95.2 & 84.0 & 92.6 & & &\\
English & 91.4 & 70.1 & 74.0 & & &\\
Greek & 86.4 & 72.0 & 86.0 & & &\\
Hebrew & 94.0 & 90.7 & 91.4 & & &\\
Japanese & 93.6 & 89.2 & 82.6 & & &\\
Korean & 97.4 & 93.5 & 94.0 & & &\\
Russian & 89.8 & 77.0 & 75.0 & & &\\
Thai & 98.0 & 92.7 & 86.4 & & &\\
Tibetan & 99.6 & 98.3 & 98.0 & & &\\ \hline
Average & 94.4 & 87.6 & 88.7 & & &\\

\hline
\end{tabular}
\end{table}

